Talking Point based Ideological Discourse Analysis in News Events

Analyzing ideological discourse even in the age of LLMs remains a challenge, as these models often struggle to capture the key elements that shape real-world narratives. Specifically, LLMs fail to focus on characteristic elements driving dominant discourses and lack the ability to integrate contextual information required for understanding abstract ideological views. To address these limitations, we propose a framework motivated by the theory of ideological discourse analysis to analyze news articles related to real-world events. Our framework represents the news articles using a relational structure - talking points, which captures the interaction between entities, their roles, and media frames along with a topic of discussion. It then constructs a vocabulary of repeating themes - prominent talking points, that are used to generate ideology-specific viewpoints (or partisan perspectives). We evaluate our framework's ability to generate these perspectives through automated tasks - ideology and partisan classification tasks, supplemented by human validation. Additionally, we demonstrate straightforward applicability of our framework in creating event snapshots, a visual way of interpreting event discourse. We release resulting dataset and model to the community to support further research.

==> qualitativeEval.tex <==
Using Fig.~\ref{fig:partisan_narrative_visualization}, we show a simple applicability of how our framework can be used for analyzing different aspects of political discourse for an event related to the Coronavirus - \textit{Biden's COVID-19 Relief Bill}. Each talking point (circle) is placed on the X-axis based on how one sided it is, based on the proportion of instances associated with each side of the political map, an equal split landing that talking point at the center. A high degree of frequent talking points with high positive or negative x-axis values, is evidence for "different realities", i.e., focusing on very different aspects of each topic. This allows us to analyze talking points by categorizing them into different types such as \textit{agreement, disagreement, one-sided etc}. Tab.~\ref{tab:narrativeViewTable} shows an instance of the same. More details on plot construction can be found in ~\ref{subsec:visualPartisanNarrative}.

% Fig.~\ref{fig:partisan_narrative_visualization} shows the prominent point distribution for an event related to the Coronavirus - \textit{Biden's COVID-19 Relief Bill}. More details on constructing the visual can be found in~\ref{subsec:visualPartisanNarrative}. We note that the high frequency talking points that are closer to Y-axis indicate that both political parties often talk about that point. In addition, farther the points are from the Y-axis, the points tend to be more specific to a particular ideology or a political party. The points above X-axis indicate agreement, and the points below indicate disagreement between the political ideologies. 

% Upon visualizing Fig.~\ref{fig:partisan_narrative_visualization}, we can categorize the talking points into four types (apart from one-sided points), and understand the narrative better. Tab.~\ref{tab:narrativeViewTable} shows an instance of the same. \textcolor{red}{maybe need better writing here.. but space is too less.}

% \begin{figure}[t!]
%   \centering
%   \includegraphics[scale=0.19]{Figures/talking_point_prominence.pdf}
%   \caption{\small Shows talking point prominence vs. points agreed/disagreed vs. partisan proportion (for an event related to Coronavirus).}
%   \label{fig:partisan_narrative_visualization}
%   \vspace{-15pt}
% \end{figure}


% \begin{table}[]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{ccll}
% \hline
% \multicolumn{1}{l}{\textbf{TP Type}} & \textbf{TP ID} & \multicolumn{1}{c}{\textbf{Left View (only titles)}}                                                                               & \multicolumn{1}{c}{\textbf{Right View (only titles)}}                                                                                  \\ \hline
% Agreement                            & 1              & Rejection of splitting COVID relief bill into separate components                & Resistance to breaking down relief package into separate bills                                                                           \\ \hline
% Disagreement                         & 10             & Emphasis on Transparency and Improved Vaccine Distribution                                                                         & Questioning Biden's Vaccine Distribution Transparency                                                                                  \\ \hline
% Agenda Setting                       & 16             & Biden's Travel Restrictions and Bans for Public Health                                                                             & \begin{tabular}[c]{@{}l@{}}Criticism of Biden's Executive Order on Pandemic Language\\ (for banning term - 'China Virus')\end{tabular} \\ \hline
% Partisan Battle                      & 2              & \begin{tabular}[c]{@{}l@{}}Biden administration's emphasis on equitable \\ vaccine distribution and healthcare reform\end{tabular} & \begin{tabular}[c]{@{}l@{}}Criticism of Biden administration's vaccine distribution \\ decisions\end{tabular}                          \\ \hline
% Right Only                           & 3              & \multicolumn{1}{c}{-}                                                                                                              & Economic Impact of \$15 Minimum Wage                                                                                                   \\ \hline
% \end{tabular}%
% }
% \caption{Overview of the talking points (TPs) based on its potential type.}
% \label{tab:narrativeViewTable}
% \end{table}

% \begin{table}[]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{ccll}
% \hline
% \multicolumn{1}{l}{\textbf{\small TP Type}} & \textbf{\small TP ID} & \multicolumn{1}{c}{\textbf{\small Left View (only titles)}}                                    & \multicolumn{1}{c}{\textbf{\small Right View (only titles)}}                                                                                  \\ \hline
% \small Agreement                            & \small 7              & \small Partisan Divide Over Budget Reconciliation for COVID Relief Bill Passage                & \small Resistance to White House stance on relief package splitting                                                                           \\
% \small Disagreement                         & \small 10             & \small Emphasis on Transparency and Improved Vaccine Distribution                              & \small Questioning Biden's Vaccine Distribution Transparency                                                                                  \\
% \small Agenda Setting                       & \small 16             & \small Biden's Travel Restrictions and Bans for Public Health                                  & \begin{tabular}[c]{@{}l@{}}\small Criticism of Biden's Executive Order on Pandemic Language\\ (\small for banning term - 'China Virus')\end{tabular} \\
% \small Partisan Battle                      & \small 2              & \small Biden administration's emphasis on equitable vaccine distribution and healthcare reform & Criticism of Biden administration's vaccine distribution decisions                                                                     \\
% \small Right Only                           & \small 3              & \multicolumn{1}{c}{-}                                                                   & \small Economic Impact of \$15 Minimum Wage                                                                                                   \\ \hline
% \end{tabular}%
% }
% \caption{Overview of the talking points (TPs) based on its potential type.}
% \label{tab:narrativeViewTable}
% \end{table}



==> scratch.tex <==
% \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Abortion}}}             & \multicolumn{1}{l|}{Ideology classifier (chatGPT)} & 76.59 & 69.59 & 67.92 \\
% \multicolumn{1}{c|}{} &
%   \multicolumn{1}{l|}{Our Partisan View} &
%   85.56 &
%   83.48 &
%   \textbf{83.48} \\
% \multicolumn{1}{c|}{} &
%   \multicolumn{1}{l|}{Our Partisan View + Metadata} &
%   83.65 &
%   80.70 &
%   80.57 \\ \midrule
% \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Gun Control}}} &
%   \multicolumn{1}{l|}{Ideology classifier (chatGPT)} &
%   75 &
%   81.25 &
%   71.79 \\
% \multicolumn{1}{c|}{} &
%   \multicolumn{1}{l|}{Our Partisan View} &
%   75 &
%   81.25 &
%   71.79 \\
% \multicolumn{1}{c|}{} &
%   \multicolumn{1}{l|}{Our Partisan View + Metadata} &
%   75 &
%   81.25 &
%   71.79 \bottomrule
